Mean-field inference methods for neural networks

Machine learning algorithms relying on deep neural networks recently allowed a great leap forward in artificial intelligence. Despite the popularity of their applications, the efficiency of these algorithms remains largely unexplained from a theoretical point of view. The mathematical description of learning problems involves very large collections of interacting random variables, difficult to handle analytically as well as numerically. This complexity is precisely the object of study of statistical physics. Its mission, originally pointed towards natural systems, is to understand how macroscopic behaviors arise from microscopic laws. Mean-field methods are one type of approximation strategy developed in this view. We review a selection of classical mean-field methods and recent progress relevant for inference in neural networks. In particular, we remind the principles of derivations of high-temperature expansions, the replica method and message passing algorithms, highlighting their equivalences and complementarities. We also provide references for past and current directions of research on neural networks relying on mean-field methods.

==> chap1.tex <==
\newpage

\section[Machine learning with neural networks
% \\ {\small (Context and motivation)}
]{Machine learning with neural networks 
% \\ {\small (Context and motivation)}
}
\label{sec:chap1}

% \addcontentsline{toc}{section}{Machine learning with Neural networks and Mean-field approximations -Context, Motivation and Scope}%

This \citechap~provides the fundamental concepts in machine learning that will be used throughout this thesis. A comprehensive reference is \cite{Goodfellow2016}. We also take this \citechap~as an opportunity to introduce the current challenges in the understanding of deep learning.  

\input{chap1_ml.tex}


